Discrete Morse theory and classifying spaces

The aim of this paper is to develop a refinement of Forman's discrete Morse theory. To an acyclic partial matching $\mu$ on a finite regular CW complex $X$, Forman introduced a discrete analogue of gradient flows. Although Forman's gradient flow has been proved to be useful in practical computations of homology groups, it is not sufficient to recover the homotopy type of $X$. Forman also proved the existence of a CW complex which is homotopy equivalent to $X$ and whose cells are in one-to-one correspondence with the critical cells of $\mu$, but the construction is ad hoc and does not have a combinatorial description. By relaxing the definition of Forman's gradient flows, we introduce the notion of flow paths, which contains enough information to reconstruct the homotopy type of $X$, while retaining a combinatorial description. The critical difference from Forman's gradient flows is the existence of a partial order on the set of flow paths, from which a $2$-category $C(\mu)$ is constructed. It is shown that the classifying space of $C(\mu)$ is homotopy equivalent to $X$ by using homotopy theory of $2$-categories. This result can be also regarded as a discrete analogue of the unpublished work of Cohen, Jones, and Segal on Morse theory in early 90's.

==> plain_category.tex <==
\subsection{Small Categories}
\label{plain_category}

Let us first fix notation and terminology for categories and
functors. We regard a small category as a monoid in the category of
quivers. 

\begin{definition} \hspace{\fill}
\begin{enumerate}
 \item  A \emph{quiver} $Q$ consists of a set $Q_0$ of vertices and a
	set $Q_1$ of arrows together with maps
	\[
	s,t : Q_1 \longrightarrow Q_0.
	\]
	For $x,y\in Q_0$ and $u\in Q_1$, when $s(u)=x$ and $t(u)=y$, we
	write $u : x\to y$. By definition, the set of arrows from $x$ to $y$ 
	equals $s^{-1}(x)\cap t^{-1}(y)$ and is denoted by $Q(x,y)$.

 \item For a quiver $Q$, define
       \[
	N_2(Q) = \set{(u,v)\in Q_1^2}{s(u)=t(v)}.
       \]

 \item A \emph{small category} is a quiver $C$ equipped with maps
       \begin{eqnarray*}
	\circ & : & N_2(C) \longrightarrow C_1 \\
	\iota & : & C_0 \longrightarrow C_1
       \end{eqnarray*}
       satisfying the associativity and the unit conditions, i.e.
       \begin{eqnarray*}
	(u\circ v)\circ w & = & u\circ(v\circ w) \\
	u & = & \iota(t(u))\circ u = u\circ \iota(s(u))
       \end{eqnarray*}
       for all $u,v,w\in C_1$ with $s(u)=t(v)$ and $s(v)=t(w)$.
       We also require that $s(u\circ v)=s(v)$, $t(u\circ v)=t(u)$, and
       $s(\iota(x))=t(\iota(x))=x$. 
       
       For $x\in C_0$, $\iota(x)$ is denoted by $1_x$ and is called the
       \emph{identity morphism} at $x$.

 \item A \emph{functor} $f$ from a category $C$ to $D$ is a pair of maps
       \begin{eqnarray*}
	f_0 & : & C_0 \longrightarrow D_0 \\
	f_1 & : & C_1 \longrightarrow D_1
       \end{eqnarray*}
       that are compatible with $s$, $t$, $\circ$, and $\iota$, i.e.\
       the following diagram is commutative
       \[
	\begin{diagram}
	 \node{} \node{C_0} \arrow[2]{e,t}{f_0} \node{} \node{D_0}
	 \\ 
	 \node{} \node{} \node{C_0} \arrow{e,-} \arrow{sw,t}{\iota} \node{}
	 \arrow{e,t}{f_0} \node{D_0} \arrow{sw,b}{\iota} \\
	 \node{} \node{C_1} \arrow[2]{e,t}{f_1} \arrow{s,-} \arrow[2]{n,l}{s}
	 \node{} 
	 \node{D_1} \arrow[2]{s,r}{t}
	 \arrow[2]{n,r}{\raisebox{-12pt}{$\scriptstyle s$}} \\ 
	 \node{N_2(C)} \arrow[2]{e,t}{N_2(f)} \arrow{ne,t}{\circ}
	 \node{\makebox[1ex]{\rule[5pt]{0pt}{13pt}}} \arrow{s,l}{t} 
	 \node{N_2(D)} 
	 \arrow{ne,b}{\circ} \\ 
	 \node{} \node{C_0} \arrow[2]{e,t}{f_0} \node{} \node{D_0.}
	\end{diagram}
       \]
 \item For functors $f,g : C\to D$, a \emph{natural transformation}
       $\theta$ from $f$ to $g$ is a map
       \[
	\theta : C_0 \longrightarrow D_1
       \]
       satisfying the following conditions:
       \begin{enumerate}
	\item $\theta(x) \in D(f(x),g(x))$ for all $x\in C_0$.
	\item The following diagram is commutative in $D$ for any
	      $u\in C(x,y)$ 
	      \[
	      \begin{diagram}
	       \node{f(x)} \arrow{s,l}{\theta(x)} \arrow{e,t}{f(u)}
	       \node{f(y)} \arrow{s,r}{\theta(y)} \\ 
	       \node{g(x)} \arrow{e,t}{g(u)} \node{g(y).}
	      \end{diagram}
	      \]
       \end{enumerate}
       In this case, we write
       \[
	\theta : f \Longrightarrow g.
       \]

 \item A category $C$ is said to be \emph{acyclic} if either $C(x,y)$ or
       $C(y,x)$ is empty for any $x, y\in C_0$ with $x\neq y$ and
       $C(x,x)=\{1_x\}$ for any 
       $x\in C_0$.
\end{enumerate}
\end{definition}

\begin{remark}
 A poset is a typical example of an acyclic category. Many of
 properties and constructions for posets can be extended to acyclic
 categories. 
\end{remark}

For a small category $C$, we have a coproduct decomposition
\[
 C_1 = \coprod_{x,y\in C_0} C(x,y).
\]
Thus a small category $C$ can be defined as a collection of a set $C_0$,
a family of sets $\{C(x,y)\}_{x,y\in C_0}$, maps 
\[
 \circ : C(y,z)\times C(x,y) \longrightarrow C(x,z),
\]
and elements $1_x\in C(x,x)$ satisfying the associativity and the unit
conditions. 

In order to study higher structures, we need categories whose sets of
morphisms $C(x,y)$ are topological spaces, posets, small categories, and
so on. More generally, there is a notion of 
categories enriched over a monoidal category. Recall that, roughly
speaking, a monoidal category is a category equipped with a ``tensor
product operation'' for pairs of objects.

\begin{definition}
 \label{enriched}
 Let $(\bm{V},\otimes, 1)$ be a strict monoidal category\footnote{It is
 well-known that any monoidal category can be replaced by a strict one.
 See Mac\,Lane's book \cite{MacLaneCategory} or Kassel's book
 \cite{KasselBook}, for example.}. 
 \begin{enumerate}
  \item A \emph{$\bm{V}$-quiver} $Q$ consists of a set $Q_0$ of vertices 
	and a family $\{Q(x,y)\}_{x,y\in Q_0}$ of objects in $\bm{V}$.
  \item A \emph{category enriched over $\bm{V}$} or simply a
	\emph{$\bm{V}$-category} consists of a $\bm{V}$-quiver $C$
	together with
	\begin{itemize}
	 \item a morphism
	       \[
	       \circ : C(y,z)\otimes C(x,y) \longrightarrow C(x,z)
	       \]
	       in $\bm{V}$ for each triple $x,y,z\in C_o$ and
	 \item a morphism $1_x:1\to C(x,x)$ in $\bm{V}$ for each $x\in C_0$
	\end{itemize}
	that are subject to the standard requirements of being a small
	category. 
 \end{enumerate}
\end{definition}

\begin{remark}
 See Kelly's book \cite{KellyEnrichedCategory_reprint} for details on
 enriched category theory.
\end{remark}

Examples of monoidal categories include the category $\Posets$ of posets,
the category $\Spaces$ of topological spaces, and the category $\Cats$ of
small categories. Monoidal structures are given by products in all of
these categories. We use the following terminologies. 

\begin{definition}
 \label{popular_enriched_categories}
 Categories enriched over $\Posets$, $\Spaces$ and $\Cats$ are called
 \emph{poset-categories}, \emph{topological categories}, and 
 \emph{(strict) $2$-categories} respectively.
\end{definition}

Note that under the inclusion $\Posets\subset\Cats$, poset-categories
can be regarded as $2$-categories.

\begin{definition}
 \label{V-functor}
 For $\bm{V}$-categories $C$ and $D$, a \emph{$\bm{V}$-functor} $f$ from
 $C$ to $D$ consists of a map
 \[
  f_0 : C_0 \longrightarrow D_0
 \]
 and a family of morphisms
 \[
  f(x,y) : C(x,y) \longrightarrow D(f_0(x),f_0(y))
 \]
 that preserve compositions and the identity morphsims.
\end{definition}

\begin{lemma}
 For a monoidal category $\bm{V}$, $\bm{V}$-categories and
 $\bm{V}$-functors form a category, denoted by $\enriched{\bm{V}}$.
\end{lemma}

For the following particular choices of $\bm{V}$, we use special names
for $\bm{V}$-functors:
\begin{itemize}
 \item When $\bm{V}=\Spaces$, $\bm{V}$-functors are called
       \emph{continuous functors}.
 \item When $\bm{V}=\Posets$, $\bm{V}$-functors are called
       \emph{poset-functors}. 
 \item When $\bm{V}=\Cats$, $\bm{V}$-functors are called \emph{(strict)
       $2$-functors}. $\enriched{\Cats}$ is denoted by $\Cats_2$.
\end{itemize}

Our first task in this paper is to construct a poset-category $C(f)$
from a discrete Morse function $f$. Since poset-categories are
$2$-categories, we need to recall basic definitions and properties of
$2$-categories.
% Throughout this section, let $\bm{V}$ be a fixed strict 
% monoidal category with initial object $1$. 
% We review the following terminology for $2$-categories.
%
%Recall that we have defined a $2$-category $C$ as a category enriched
%over the category $\Cats$ of small categories in Definition
%\ref{popular_enriched_categories}. Another way of understanding a
%$2$-category is to regard it as a $2$-quiver with compositions.

%\begin{definition}
% When $\Quivers$ is the category of quivers, $\Quivers$-quivers
% are called \emph{$2$-quivers}. For a $2$-quiver $Q$ and a pair of
% vertices $x,y\in Q_0$, elements of $Q(x,y)_0$ and $Q(x,y)_1$ are called 
% \emph{$1$-arrows} and \emph{$2$-arrows}.
%\end{definition}

%Thus a $2$-category is a $2$-quiver $C$ equipped with ``compositions''
%\begin{eqnarray*}
% \circ & : & C(y,z)\times C(x,y) \rarrow{} C(x,z) \\
% * & : & C(x,y)(v,w)\times C(x,y)(u,v) \rarrow{} C(x,y)(u,w)
%\end{eqnarray*}
%satisfying the associativity and the unit conditions, for $x,y,z\in C_0$
%and $u,v,w\in C(x,y)_0$. With this in mind, we used the following
%terminology. 

 For a $2$-category $C$ and objects $x,y\in C_0$, $C(x,y)$ is a small
 category. Thus it consists of the set of objects $C(x,y)_0$
 and morphisms $C(x,y)_1$. Elements of $C(x,y)_0$ and $C(x,y)_1$ are
 called \emph{$1$-morphisms} and \emph{$2$-morphisms} in $C$,
 respectively. When $\theta\in C(x,y)(u,v)$, we 
 write $\theta : u\Rightarrow v$.

 The classes of all $1$-morphisms and
 $2$-morphisms in $C$ are denoted by $C_1$ and $C_2$, respectively. When 
 $C_2$ is a set, $C$ is called a \emph{small} $2$-category.

 There are two kinds of compositions in a $2$-category
 $C$. First of all, given a triple $x,y,z\in C_0$ of objects, we have
 the \emph{horizontal composition} functor
 \[
 \circ : C(y,z)\times C(x,y) \longrightarrow C(x,z).
 \]
 On the other hand, for a triple $u,v,w\in C(x,y)_0$, we have the
 \emph{vertical composition} denoted by
 \[
 \ast : C(x,y)(v,w)\times C(x,y)(u,v) \longrightarrow C(x,y)(u,w).
 \]
% Thus, for $1$-morphisms, we only have $\circ$. But for $2$-morphisms,
% we have two kinds of composition operations.

\begin{remark}
 Any category can be made into a $2$-category by adding
 identity $2$-morphisms.
 In the rest of this paper, such $2$-categories coming from ordinary
 categories are called \emph{$1$-categories}. 
\end{remark}

There are weaker versions of $2$-categories such as bicategories and
$(\infty,2)$-categories. In this paper, we only use strict
$2$-categories. 
For the sake of simplicity, strict $2$-categories are simply called
$2$-categories throughout the rest of this paper.

%\begin{definition}
% A $\Cats$-functor $f:C\to D$ between $2$-categories is called
% a\emph{$2$-functor}. 
%\end{definition}

Even though we only use strict $2$-categories, 
we are often forced to use weaker notions of functors between
$2$-categories. 

\begin{definition}
 \label{lax_functor_definition}
 Let $C$ and $D$ be small $2$-categories.
 A \emph{lax functor} $f$ from $C$ to $D$
 consists of the following data:
 \begin{itemize}
  \item a map
	\[
	 f : C_0 \longrightarrow D_0,
	\]
  \item a family of functors
	\[
	 f=f_{y,x} : C(x,y) \longrightarrow D(f(x),f(y)),
	\]
  \item a family of natural transformations
	\[
	\xymatrix{%
	f(x) \ar[r]^{f(w)}
	\rruppertwocell<15>^{f(w'\circ w)}{\omit}
	& f(x') \ar[r]^{f(w')} & f(x'')
	\lltwocell<\omit>{<4>\hspace*{50pt}f_{x'',x',x}}
	}
	\]
  \item a family of natural transformations 
	\[
	\xymatrix{%
	f(x) \rtwocell^{1_{f(x)}}_{f(1_x)}{f_x} & f(x).
	}
	\]
 \end{itemize}
 These maps must satisfy the following additional conditions: 
 \begin{enumerate}
  \item The following diagram is commutative in $D(f(x),f(t))$
	
	\begin{equation}
	\xymatrixcolsep{45pt}
	 \xymatrix{
	(f(w)\circ f(v))\circ f(u) \ar@{=}[d]
	\ar@{=>}[r]^(0.55){f_{q,z,y}\circ 1_{f(u)}} & f(w\circ v)\circ f(u)
	\ar@{=>}[r]^{f_{q,y,x}} & f((w\circ v)\circ u) \ar@{=}[d] \\
	f(w)\circ (f(v)\circ f(u))
	\ar@{=>}[r]_(0.55){1_{f(w)}\circ f_{z,y,x}} &
	f(w)\circ f(v\circ u) \ar@{=>}[r]_{f_{q,z,x}} &
	f(w\circ(v\circ u)) 
	}
	\label{composer}
	\end{equation}
	for any composable $1$-morphisms
	$x \rarrow{u} y \rarrow{v} z \rarrow{w} q$ in $C$.

  \item The following diagrams are commutative in $D(f(x),f(y))$
	\begin{equation}
	\xymatrixcolsep{30pt}
	\xymatrix{ 
	f(u)\circ 1_{f(x)} \ar@{=}[d] \ar@{=>}[r]^{1_{f(u)}\circ f_x} &
	f(u)\circ f(1_x) \ar@{=>}[r]^(0.54){f_{y,x,x}} & f(u\circ 1_x)
	\ar@{=}[d] \\ 
	f(u) \ar@{=}[rr] & & f(u)
	}
	\label{uniter1}
	\end{equation}
	\begin{equation}
	\xymatrixcolsep{30pt}
	\xymatrix{
	1_{f(y)}\circ f(u) \ar@{=}[d] \ar@{=>}[r]^{f_y\circ 1_{f(u)}} & 
	f(1_y)\circ f_1(u) \ar@{=>}[r]^(0.54){f_{y,y,x}} & f(1_y\circ u)
	\ar@{=}[d] \\ 
	f(u) \ar@{=}[rr] & & f(u)
	}
	\label{uniter2}
	\end{equation}
	for any $1$-morphism $u : x\to y$ in $C$.
 \end{enumerate}

 $f$ is called a \emph{normal lax functor} when $f_x$ is the identity
 for all objects $x \in C_0$.  
\end{definition}

\begin{remark}
 For simplicity, we suppress the indices in $f_{z,y,x}$ and $f_x$ and
 denote them by $f$, when there is no danger of confusion.
\end{remark}

\begin{remark}
 \label{colax_functor_definition}
 We may reverse the directions of natural transformations $f_{x,y,z}$
 and $f_x$ to obtain the notion of \emph{colax functors}. In fact, 
 one of the most important tools in this paper is a colax functor,
 the \emph{collapsing functor} $\tau$, constructed in
 \S\ref{collapsing_functor} . 

 Note that colax functors are often called \emph{oplax functors} in the
 literature. The choice of the term ``colax'' is based on the general
 principle that, when $2$-morphisms are reversed, we put a suffix
 ``co''. 

 When these natural transformations are isomorphisms, $f$ is
 called a \emph{pseudofunctor}. In particular, a pseudofunctor can be
 regarded as a lax functor and a colax functor.
\end{remark}

\begin{lemma}
 $2$-categories and lax functors form a category, denoted by
 $\Cats_{2,l}$. Normal lax functors form a subcategory, denoted by
 $\Cats_{2,nl}$. We also obtain the category of $2$-categories and colax
 functors $\Cats_{2,cl}$ and its subcategory of normal colax functors
 $\Cats_{2,ncl}$. 
\end{lemma}

\begin{proof}
 We only verify the case of lax functors.
 The composition of lax functors
 \[
  B \rarrow{f} C \rarrow{g} D
 \]
 is defined by the composition 
 \[
 B_0 \rarrow{f} C_0 \rarrow{g} D_0
 \]
 on objects and the composition
 \[
 B(x,y) \rarrow{f_{x,y}} C(f(x),f(y)) \rarrow{g_{f(x),f(y)}}
 D(g(f(x)),g(f(y))) 
 \]
 on 1-morphisms. For a triple $x,y,z\in B_0$, the natural transformation
 $(g\circ f)_{z,y,x}$ is
 given by the composition of natural transformations
 \[
 \xymatrixcolsep{55pt}
 \xymatrix{
 B(y,z)\times B(x,y) \ar[d]_{f_{z,y}\times f_{y,x}} \ar[r]^{\circ} &
 B(x,z) \ar[d]^{f_{z,x}} \\ 
 C(f(y),f(z))\times C(f(x),f(y)) \ar@{=>}[ur]^{f_{z,y,x}}
 \ar[d]_{g_{f(z),f(y)}\times g_{f(y),f(x)}} \ar[r]^(0.6){\circ} &
 C(f(x),f(z)) \ar[d]^{g_{f(z),f(x)}} \\  
 D(g(f(y)),g(f(z)))\times D(g(f(x)),g(f(y)))
 \ar@{=>}[ur]^{g_{f(z),f(y),f(x)}} \ar[r]^(0.63){\circ} &
 D(g(f(x)),g(f(z))). 
 }
 \]
 Finally the natural transformation $(g\circ f)_x$ is defined by the
 composition
 \[
 \xymatrixcolsep{60pt}
 \xymatrix{
 I \ar@{=}[d] \ar[r]^{\iota(x)} & B(x,x) \ar[d]^{f_{x,x}} \\
 I \ar@{=>}[ur]^{f_x} \ar@{=}[d] \ar[r]^{\iota(f(x))} & C(f(x),f(x))
 \ar[d]^{g_{f(x),f(x)}} \\ 
 I \ar@{=>}[ur]^{g_{f(x)}} \ar[r]_(0.38){\iota(g(f(x)))} &
 D(g(f(x)),g(f(x))). 
 }
 \]
 Since the composition is defined by compositions of maps and natural
 transformations, it is associative.
 The identity (lax) functor $1_{B}: B\to B$ serves as a unit and we
 obtain a category $\Cats_{2,l}$.
\end{proof}

